ProtoQA: A Question Answering Dataset for Prototypical Common-Sense Reasoning

Given questions regarding some prototypical situation such as Name something that people usually do before they leave the house for work? a human can easily answer them via acquired experiences. There can be multiple right answers for such questions, with some more common for a situation than others. This paper introduces a new question answering dataset for training and evaluating common sense reasoning capabilities of artificial intelligence systems in such prototypical situations. The training set is gathered from an existing set of questions played in a long-running international game show FAMILY- FEUD. The hidden evaluation set is created by gathering answers for each question from 100 crowd-workers. We also propose a generative evaluation task where a model has to output a ranked list of answers, ideally covering all prototypical answers for a question. After presenting multiple competitive baseline models, we find that human performance still exceeds model scores on all evaluation metrics with a meaningful gap, supporting the challenging nature of the task.

==> sections/analysissectionfigure.tex <==

\begin{figure}\begin{tikzpicture}
\begin{axis}[
  xmax=10,
  ybar,
  bar width=0.2cm,
  xlabel=Numbers of answer clusters per question,
  legend pos=north west
]
    
        \addplot[
    color=blue
    ]
    coordinates { (1, 0.011224489795918367) (2, 0.09795918367346938) (3, 0.03163265306122449) (4, 0.22755102040816327) (5, 0.2714285714285714) (6, 0.2571428571428571) (7, 0.0836734693877551) (8, 0.01020408163265306) (9, 0.0010204081632653062) (11, 0.0010204081632653062) 
    };
      
    

            \addplot[
    color=red
    ]
    coordinates {(1, 0.023529411764705882) (2, 0.023529411764705882) (3, 0.052941176470588235) (4, 0.11176470588235295) (5, 0.11764705882352941) (6, 0.21764705882352942) (7, 0.18235294117647058) (8, 0.1588235294117647) (9, 0.06470588235294118) (10, 0.029411764705882353) (11, 0.01764705882352941)
    };
    

    \legend{Train, Collected}
 
\end{axis}
\end{tikzpicture}
\caption{\label{datadist}Number of answer clusters per question, in the scraped (blue) and crowdsourced (red) datasets. }
\end{figure}



==> sections/continuouseval.tex <==
\subsection{Continuous Human Evaluation}
\label{sub:cont_human_eval}

Even though the answer to each \ff test question have been crowd-sourced from 100 annotators, there is still a possibility that our automatic evaluation strategy wrongly penalizes a model because the predicted answer is not present in the collected list of answers. To tackle this problem, we propose the evaluation of model predictions as another crowd-sourcing task as follows (figure~\ref{fig:mockup_human_eval}).
\begin{itemize}
    \item Any model prediction that does not exactly match with the list of answers will be sent to the crowd sourcing task.
    \item Along with the model prediction, the crowd workers will be shown the question and the clusters of existing answer. The worker will then decide which cluster does the prediction belong to and would assign the answer to that cluster.
    \item If the answer is a correct / reasonable w.r.t to the question but does not closely resemble any cluster, then the worker can create a new cluster and assign it there. However, if the answer is clearly wrong or unrelated to the question, then the worker can mark it as a wrong/invalid answer.
    \item Each cluster is associated with a popularity score which is defined as proportion of answers (collected in the initial crowd-sourcing phase) that belong to that cluster. For example, if answers of 70 crowd-workers belong to the ``breakfast'' cluster, then the popularity of that cluster is 0.7. Now if a new answer is assigned to this cluster, then the score of that prediction is proportional to the popularity. If a new cluster is created for an answer, we assign it a low popularity score of \raj{0.01}.
\end{itemize}

This evaluation paradigm addresses the long-standing challenge of open-domain evaluation of NLP tasks. However, the main drawback of this approach is that this evaluation paradigm is slower than the automated approaches. Currently, a batch of 10 questions take \raj{5 minutes} to be replicated by \raj{3 workers} and cost us \raj{2 USD}. \raj{This is a lot cheaper than re-creating an entire benchmark dataset as it is solved.}

\subsubsection{Discussion}
\begin{itemize}
    \item 1. Will each question be annotated by multiple workers?
    \item 2. How much is this going to cost per model? Is the cost reasonable?
    \item 3. What is a good estimate of time? Would we update our leader board monthly?, one week before every *CL conference deadline?
\end{itemize}



==> sections/futurework.tex <==
In addition to the elements of this task which are appealing from a common sense modeling perspective, the inherent appeal of this task to humans opens a number of possibilities for future data collection and evaluation.  While the high availability of crowdsource workers has led to great progress in dataset generation it is not without its flaws, and weeding out poor quality responses is often non-trivial for more interesting tasks. On the other hand, millions of people play this game as an app on their phones\footnote{\url{http://shorturl.at/lnoEZ}}, not for any monetary gain but simply for their own enjoyment. In the future we propose to collect more data by creating a form of this game, leveraging people's natural interest and enjoyment and using mechanism design to encourage high quality answers to more common sense questions.
% The framework of such an app would also allow for fast and accurate human evaluation of model outputs, supplementing automatic evaluation methods for a more accurate assessment of models.

==> sections/perturbation_rules.tex <==
Perturbation method works as follows.  
\begin{enumerate}
    \item A question-maker examines a question from a list of 2800 un-answered questions (so that the original question is similar to the training set)
    \item Question-maker attempts to make a minimal perturbation to the question -- looking at changing the entities or events mentioned in the text -- which would both maintain the intuitions required of hte question but change the actual answers.
    \item If such a perturbation is not possible without reducing the common-sense nature of the question, question-maker attempts to see whether changes to any two parts of the question can derive a question with similar characteristics. 
    \item Question-makers are allowed to skip questions if they cannot create any perturbed version of a given question (report rates here)
    \item All questions are then given ratings 1-5 by at least one question-maker (maybe two?), summarizing the combination of whether the question assesses challenging common-sense reasoning, and whether the question is similar in nature and quality to the training dataset. 
    \item 300 questions in total were generated, and the 250 with highest scores chosen. [Report agreement here].
    \end{enumerate}
\textit{Ideally, I'd like to tweak this according to whatever we want to do long-term regarding crowd-sourcing of questions, so that we can, in the future, use this a starting point. }

==> sections/scoring_perturbed_questions.tex <==
This is the standard of a 5 scored question in out scoring system to determine whether this is a good question.
\begin{enumerate}
    \item Most humans are expected to know
    \item The answer set is relative small answer set, less than 8 big categories of different answers.
    \item The question is hard for system relying on co-occurrence patterns to answer, e.g Bert
    \item The question is precise, not too ambiguous. e.g Name a country where you would find cactus.
    \item The answers are not be different for people with different background, e.g Name a dish made with ground meat. Chinese would have totally different answer set compared to American.
    \item To answer this question, multi-step reasoning is needed based on commonsense reasoning. E.g If You Were Stranded With Other People On An Island, Which Useful Occupations Would You Want Them To Have?
    \end{enumerate}

\begin{figure*}
\centering
\includegraphics[width=2\columnwidth]{images/mockup_human_eval_interface.pdf}
\caption{Mockup for the human evaluation interface. Annotators can drag the predicted answer to any one of the already existing clusters that closely resembles the answer. If the answer is clearly wrong, they can mark it as invalid. If the answer does not fit into any given category, then a new cluster can be created. Predictions are scored based on the popularity of  the assigned cluster (see text for details about popularity of a cluster).}
\label{fig:mockup_human_eval}
\end{figure*}

==> sections/test_question_generation.tex <==
For confirming annotator quality, test questions were selected to maximize two conflicting goals, of both being very similar to the primary task while also having a small finite set of possible answers.  A focus was placed upon questions wherein a very casual reading would result in incorrect answers. 
